A Bitstream Feature Based Model for Video Decoding Energy Estimation

In this paper we show that a small amount of bit stream features can be used to accurately estimate the energy consumption of state-of-the-art software and hardware accelerated decoder implementations for four different video codecs. By testing the estimation performance on HEVC, H.264, H.263, and VP9 we show that the proposed model can be used for any hybrid video codec. We test our approach on a high amount of different test sequences to prove the general validity. We show that less than 20 features are sufficient to obtain mean estimation errors that are smaller than 8%. Finally, an example will show the performance trade-offs in terms of rate, distortion, and decoding energy for all tested codecs.

==> gfx/distribution_energy4_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA data7}%
\psfrag{017}[cl][cl]{\matlabtextA data6}%
\psfrag{018}[cl][cl]{\matlabtextA data5}%
\psfrag{019}[cl][cl]{\matlabtextA data4}%
\psfrag{020}[cl][cl]{\matlabtextA data3}%
\psfrag{021}[cl][cl]{\matlabtextA data2}%
\psfrag{022}[cl][cl]{\matlabtextA daaaaaaaata1}%
\psfrag{023}[tc][tc]{\matlabtextA Energy}%
\psfrag{024}[tr][tr]{\matlabtextA VP9}%
\psfrag{025}[tr][tr]{\matlabtextA H.263}%
\psfrag{026}[tr][tr]{\matlabtextA H.264}%
\psfrag{027}[tr][tr]{\matlabtextA HEVC}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $0.2$}%
\psfrag{002}[ct][ct]{\matlabtextA $0.4$}%
\psfrag{003}[ct][ct]{\matlabtextA $0.6$}%
\psfrag{004}[ct][ct]{\matlabtextA $0.8$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextA $1$}%
\psfrag{006}[rc][rc]{\matlabtextA $2$}%
\psfrag{007}[rc][rc]{\matlabtextA $3$}%
\psfrag{008}[rc][rc]{\matlabtextA $4$}%
\psfrag{009}[rc][rc]{\matlabtextA $5$}%
\psfrag{010}[rc][rc]{\matlabtextA $6$}%
\psfrag{011}[rc][rc]{\matlabtextA $7$}%
\psfrag{012}[rc][rc]{\matlabtextA $8$}%
\psfrag{013}[rc][rc]{\matlabtextA $9$}%
\psfrag{014}[rc][rc]{\matlabtextA $10$}%
\psfrag{015}[rc][rc]{\matlabtextA $11$}%
%
%% </ytick>
